Towards Accurate and Reliable Energy Measurement of NLP Models

Accurate and reliable measurement of energy consumption is critical for making well-informed design choices when choosing and training large scale NLP models. In this work, we show that existing software-based energy measurements are not accurate because they do not take into account hardware differences and how resource utilization affects energy consumption. We conduct energy measurement experiments with four different models for a question answering task. We quantify the error of existing software-based energy measurements by using a hardware power meter that provides highly accurate energy measurements. Our key takeaway is the need for a more accurate energy estimation model that takes into account hardware variabilities and the non-linear relationship between resource utilization and energy consumption. We release the code and data at https://github.com/csarron/sustainlp2020-energy.

==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

Energy estimation is an important research topic in both the machine learning and system community. We discuss two threads of research related to energy measurement for NLP models:

{\bf Energy estimation in machine learning and NLP.} \cite{henderson2020SystematicReporting} uses a software framework called \textit{experiment-impact-tracker} to report the aggregated energy of the benchmark programs. The \textit{experiment-impact-tracker} collects hardware resources statistics, and uses a simple linear model~\cite{strubell2019EnergyPolicy} to estimate the total energy where the coefficients are fixed to a constant without considering the actual hardware device configurations. We have shown in the experiments that such software based energy estimation methods are not accurate nor robust. We recommend using hardware power meters to measure the energy consumption, and then possibly calibrate the software energy values. \cite{zhou2020HULKEnergy} presents an energy efficient benchmark for NLP models. However, they only report the time (hours) and cost (dollars) for training and testing NLP models, the actual energy numbers remain unknown. The ``Green AI" \cite{schwartz2019GreenAIa} work suggests using metrics like floating point operations (FPO) to measure energy efficiency, \cite{henderson2020SystematicReporting} argues such metrics alone cannot reflect model energy consumption. A recent work\cite{garcia-martin2019Estimationenergy} surveys comprehensive energy estimation methods in machine learning, while little energy results for NLP models are reported yet. 

{\bf Energy modeling for systems and applications.}
Energy estimation for battery powered devices such as mobile phones is critical since mobile applications utility can be limited by the battery life. Previous work \cite{pathak2011Finegrainedpower,pathak2012Whereenergya,yoon2012AppScopeapplication,cao2017DeconstructingEnergy} study various fine-grained system level power modeling and profiling techniques that help understand energy drain of applications. NLP models essentially power many emerging applications such as personal assistants with mobile intelligence. However, the energy implications for these NLP models are unclear, it is non-trivial to leverage system level fine-grained power modeling methods without delving deep into NLP models' unique semantics. We leave fine-grained energy modeling of NLP models as future work.


